Vapnik-Chervonenkis Dimension and Density on Johnson and Hamming Graphs

VC-dimension and VC-density are measures of combinatorial complexity of set systems. VC-dimension was first introduced in the context of statistical learning theory, and is tightly related to the sample complexity in PAC learning. VC-density is a refinement of VC-dimension. Both notions are also studied in model theory, in the context of \emph{dependent} theories. A set system that is definable by a formula of first-order logic with parameters has finite VC-dimension if and only if the formula is a dependent formula. In this paper we study the VC-dimension and the VC-density of the edge relation $Exy$ on Johnson graphs and on Hamming graphs. On a graph $G$, the set system defined by the formula $Exy$ is the vertex set of $G$ along with the collection of all \emph{open neighbourhoods} of $G$. We show that the edge relation has VC-dimension at most $4$ on Johnson graphs and at most $3$ on Hamming graphs and these bounds are optimal. We furthermore show that the VC-density of the edge relation on the class of all Johnson graphs is $2$, and on the class of all Hamming graphs the VC-density is $2$ as well. Moreover, we show that our bounds on the VC-dimension carry over to the class of all induced subgraphs of Johnson graphs, and to the class of all induced subgraphs of Hamming graphs, respectively. It also follows that the VC-dimension of the set systems of \emph{closed neighbourhoods} in Johnson graphs and Hamming graphs is bounded. Johnson graphs and Hamming graphs are well known examples of distance transitive graphs. Neither of these graph classes is nowhere dense nor is there a bound on their (local) clique-width. Our results contrast this by giving evidence of structural tameness of the graph classes.

==> Hamming/Lemmas/CliqueWidth.tex <==
\begin{theorem}
Let $d≤1$ and $q≤2$ then the Hamming graph $H(d,q)$ has clique width at least $d$.

\begin{proof}
Lemma \ref{hd0} gives us that for a given vertex $v$ in $H(d,q)$, $N(v)$ induces $d$ disjoint copies of $K_{q-1}$ with no edges between them.
For each of those cliques we choose one of its vertices $u_i$.
Since these vertices are all connected to $v$ but none of them connected to each other they are pairwise at distance $2$ from one another.
By Lemma \ref{hd2} we have that for all pairs $(u_i,u_j)$ where $1≤i<j≤q$  there is a vertex $w_{ij}$ connected to both of them.
Moreover $w_{ij}$ is not connected to $v$ so by Lemma \ref{hd2} we get that $N(w_ij)∩N(v)=\{u_i,u_j\}$ so the vertices $w_ij$ are all distinct.
Then $\{u_i|1≤i≤d\}∪\{w_ij|1≤i<j≤d\}$ induces the $1$-subdivision of $K_{d}$.
\end{proof}
\end{theorem}
\begin{corollary}
Let $d≤1$ and $q≤2$ then the Hamming graph $H(d,q)$ has clique width at least $d$.
\end{corollary}


==> Hamming/Lemmas/Lemmas.tex <==
\subsection{Properties of Hamming Graphs}

\begin{lemma}
\label{Hd1}
Let $u$ and $v$ be vertices in the Hamming Graph $H(d,q)$ with $d(u,v)=1$.

Let $1≤i≤d$ be such that $u$ and $v$ agree on all but the $i$th coordinate. % $u_i≠v_i$ and $∀k(k≠i \rightarrow u_k=v_k)$.

Then $w∈N(u)∩N(v)$ if and only if $w$ agrees with $u$ and $v$ in all but the $i$th coordinate.
%
%$$
%w≠u∧
%w≠v∧
%∀k(k≠i \rightarrow w_k=v_k=u_k)
%$$
\begin{proof}
Since $u$ and $v$ are neighbours we know that they agree in all but but one coordinate the $i$-th.
All vertices that agree with $u$ and $v$ on all coordinates except $i$-th will be in $N(u)∩N(v)$.

Take any vertex $w$ neighboring $u$ that agrees on all coordinates except the $j$-th for a $j≠i$.
Now we know that $w$ and $u$ agree on the $i$-th coordinate but since $u$ and $w$ disagree on this coordinate we 
get that $w$ and $v$ disagree on the $i$-th and the $j$-th coordinate and therefore do not have an edge between them.
Similarily any vertex neighboring $v$ that agrees with $v$ on the $i$-th coordinate will not be adjacent to $w$.

\end{proof}

\end{lemma}
\begin{lemma}
\label{Hd1q}
Let $u$ and $v$ be vertices in the Hamming graph $H(d,q)$ with $d(u,v)=1$.
Then $N(u)∩N(v)$ induces a clique of size $q-2$.
\begin{proof}
Since $u$ and $v$ are neighbours we know that there  is an $i$ such that 
$u$ and $v$ agree on all but the $i$-th coordinate.
By lemma \ref{Hd1} we know that
all of the vertices in $N(u)∩N(v)$ will also agree with $u$ and $v$ on those coordinates.
By the definition of $H(d,q)$ there are $q$ vertices that agree on all but one coordinate and those form a clique.
Neither $u$ nor $v$ are in $N(u)∩N(v)$ and therefore $N(u)∩N(v)$ induces a clique of size $q-2$.
\end{proof}
\end{lemma}

\begin{lemma}
\label{Hd2}
Let $u$ and $v$ be vertices in the Hamming Graph $H(d,q)$ with $d(u,v)=2$.
Let $1≤i<j≤d$ be such that $u_i≠v_i$ $u_j≠v_j$ and $∀k((k≠i ∧ k≠j) \rightarrow u_k=v_k)$.
Then $w∈N(u)∩N(v)$ if and only if
$$
(
	(w_i=v_i∧w_j=u_j)
	∨
	(w_i=u_i∧w_j=v_j)
)
∧
∀k((k≠i∧k≠j) \rightarrow w_k=v_k=u_k)
$$
\begin{proof}
Let $w$ be a vertex in $N(u)$ 


Since $u$ and $v$ disagree on both the $j$-th and the $i$-th coordinates any vertex $w∈N(u)∩N(v)$ 
will have to agree with $u$ on either the $i$-th or the $j$-th coordinate and with $v$ on the other one of those.


\end{proof}
\end{lemma}


\begin{lemma}
\label{Hd2q}
Let $u$ and $v$ be vertices in the Hamming graph $H(d,q)$ with $d(u,v)=2$.
Then $N(v)∩N(w)$ contains $2$ non adjacent vertices.
\begin{proof}
Let $u$ and $v$ be vertices in the Hamming graph $H(d,q)$ with $d(u,v)=2$ 
and $1≤i<j≤d$ be such that $u_i≠v_i$ and $u_j≠v_j$ 
By lemma \ref{Hd2} we know that vertices $w∈N(u)∩N(v)$ satisfy 
$$
(
	(w_i=v_i∧w_j=u_j)
	∨
	(w_i=u_i∧w_j=v_j)
)
∧
∀k((k≠i∧k≠j) \rightarrow w_k=v_k=u_k)$$
Without loss of generality assume $i=1$ and $j=2$.
It is now sufficient to show that only two vertices can satisfy this formula and that they are not adjacent.
Note that 
$(x_i)_{i=1}^d$ with $x_1=u_1$ and $∀i>1 (x_i=w_i) $
$(y_i)_{i=1}^d$ with $y_1=w_1$ and $∀i>1 (y_i=u_i) $
satisfy the formula.
They disagree in the first two coordinates so they are not adjacent.
\end{proof}
\end{lemma}

\begin{lemma}
Let $u$ and $v$ be vertices in the Hamming graph $H(d,q)$ then

$$
|N(v)∩N(w)|=%\left\{
	\begin{cases}
	d(q-1)	&\text{ if } d(u,v)=0\\
	q-2	&\text{ if } d(u,v)=1\\
	2	&\text{ if } d(u,v)=2\\
	0	&\text{ if } d(u,v)≥3
	\end{cases}	
%\right. %}
$$
\end{lemma}




==> Johnson/Density/Dugald.tex <==
\begin{theorem}
The shatter function $π(n)$ for the edge relation in $J(m,k)$ satisfies

$$π(n)≤4n+\min(m,n+1)\min(k,n+1)+π(n-1)$$

\begin{proof}
Let 
%$J(m,3)$ , with $m$ arbitrarily large.
$|A|=n$ be a set of vertices which is maximally shattered for sets of size $n$.
Let
$v∈A$
\begin{align*} 
S(A)&=\{N(u)∩A|u∈V(G)\}\\
S_1(A) &= \{ X∈ S(A): v∈X\}\\
S_2(A) &= \{ X∈ S(A): v∉X\}\\
T_1(A) &= \{ X∈ S(A): X∩N(v)≠∅\}\\
T_2(A) &= \{ X∈ S(A): X∩N(v)=∅\}\\
\end{align*}
Note that $S(A)=S_1(A)∪S_2(A)$. 
Note that $S(A)=S_1(A)∪(T_1(A)∖S_1(A))∪T_2(A)$.

%We prove the theorem by induction on $n$.
%Base case:
%We know by lemma \ref{SauerShelah} and theorem \ref{Johnson\VCDim} that $π{n}=2^n$ for  $n≤4$.
%$π(4)=2^4≤4\cdot 4^2$.

%Induction hypothesis:
%$$π(n-1)≤4(n-1)^2=4n^2-8n+4$$

%Inductive step:
Note that by our assumption that $A$ is maximally shattered we have  $|S(A)|= π(n)$.  
Since $S_2(A)=S(A∖\{v\})$ we know that $|S_2(A)|≤π(n-1)$.%as per induction hypothesis


Note that every member of  
$S_1(A)$ is an intersection of the neighbourhood of a neigbour of $v$ and $A$.
As these neighbours fully characterise each member of $S_1(A)$ we will use them evenhandedly to refer to
members of $S_1(A)$.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
We want count how many sets there are in $S_1(A)$. 
We do this by counting how many distinct neighbourhoods a given vertex in $A$ can occur in with $v$ and adding up over $A$.
This gives us a very loose upper bound which is sufficient for our purposes.
 


Let
\begin{align*} 
D_0&=\{v\}\\
D_1&=\{u∈A,d(u,v)=1\}\\
D_2&=\{u∈A,d(u,v)=2\}\\
D_3&=\{u∈A,d(u,v)=3\}
D_4&=\{u∈A,d(u,v)≥4\}
\end{align*}
Note that $⋃_{i=0}^4D_i=A$ and for $i≠j$ we have $D_i∩D_j=∅$.

Any element of $D_3$ can only belong to members of $S_2(A)$ since they have  no common neighbours with $v$.

An element of $D_2$ can be a member of at most $4$ elements of $S_1(A)$ since $v$ only shares $4$ neighbours with every element of $D_2$.
Since $D_2⊆A$ we have $|D_2|≤|A|$,
%Note that as subsets of $A$, the size of $D_2$ is linearly bounded by $|A|$.
so the total number of sets in $S_1(A)$ that intersect $D_2$ is at most $4|A|$.

It only remains to count those sets in $S_1(A)$ that intersect $A$ only in $D_1$.

Since $D_1=N(v)∩A$ and any set in $S_1(v)$ must be characterised by a vertex in $N(v)$ 
we know that the number of sets in $S_1(v)$ contained in $D_1$ is bounded above by 
the shatter function $π'(n)$ for the edge relation in the $m$ by $k$ rook graph which by Lemma \ref{rook}
is bounded by $\min(i+1,n)\min(i+1,m)$.
 
$D_0$ is a singleton and its element $v$ is common to all members of $S_1(A)$ and it can therefore not distinguish any two members of $S_1(A)$.
So it adds no new sets to $S_1(A)$ unless $D_1=D_2=∅$.

So $|S_1(A)|=4n+\min(n+1,k)\min(n+1,m)$


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%new stufff %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
We now want to compute
$|T_1(A)∖S_1(A)|$.
Note that this is those neighbourhoods that intersect $N(v)$ but do not contain $v$ so they are 

A vertex from $D_4$ can only be a member of elements of $T_2(A)$.

A vertex from $D_3$ can be a member of at most $4|D_1| $ elements of $T_1(A)$  
giving us $4|D_1||D_3|$ elements.


So it only remains to count those sets in $T_1(A)$ that intersect $A$ only in $D_1∪D_2$.

Let $X$ be such a set 
Look at those $X$ such that the diameter is $1$ and those such that the diameter is $2$





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%old stuff %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%&


 
So we  now have a bound on the size of every part of  $S_1(A)$ and can compute a bound for $S(A)$.

\begin{align*}
&π(n)=|S(A)|=\\
&|S_1(A)|+	|S_2(A)|≤\\
&0+4|A|+π'(n)+π(n-1)=\\
%&0+4|D_1|+π'(n)+π(n-1)=\\
&4n+\min(n+1,k)\min(n+1,m)+π(n-1)\\
\end{align*}

\end{proof}
\end{theorem}




==> Johnson/Density/Induction.tex <==
\begin{theorem}
The shatter function $π(n)$ for the edge relation in Johnson graphs for three sets is:

$$π(n)≤4n^2$$

\begin{proof}

Let 
$J(m,3)$ , with $m$ arbitrarily large.
$|A|=n$ be a set of vertices which is maximally shattered for sets of size $n$.
Let
\begin{align*} 
v&=\{1,2,3\}∈A\\
S(A)&=\{N(u)∩A|u∈V(G)\}\\
S_1(A) &= \{ X∈ S(A): v∈X\}\\
S_2(A) &= \{ X∈ S(A): v∉X\}\\
\end{align*}
Note that $S(A)=S_1(A)∪S_2(A)$ 


We prove the theorem by induction on $n$.
Base case:
We know by lemma \ref{SauerShelah} and theorem \ref{VC-dimTheorem} that $π(n)=2^n$ for  $n≤4$.
$π(4)=2^4≤4\cdot 4^2$.

Induction hypothesis:
$$π(n-1)≤4(n-1)^2=4n^2-8n+4$$

Inductive step:
Note that by our assumption that $A$ is maximally shattered we have  $|S(A)|= π(n)$.  
Since $S_2(A)=S(A∖\{v\})$ we know by induction hypothesis that $|S_2(A)|≤π(n-1)≤4(n-1)^2$.%as per induction hypothesis


Note that every member of  
$S_1(A)$ is an intersection of the neighbourhood of a neigbour of $v$ and $A$,
as these neighbours fully charectarise each member of $S_1(A)$ we will use them evenhandedly to refer to
members of $S_1(A)$.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
We want count how many sets there are in $S_1(A)$ we do this by counting how many distinct neighbourhoods a given vertex in $A$ can occur in with $v$ and adding up over $A$.
This gives us a very loose upper bound which is sufficient for our purposes.
 


Let
\begin{align*} 
B_1&= \{\{1,i,j\}∈A|i≠2,j≠2,i≠3,j≠3\}\\
B_2&= \{\{2,i,j\}∈A|i≠1,j≠1,i≠3,j≠3\}\\
B_3&= \{\{3,i,j\}∈A|i≠1,j≠1,i≠2,j≠2\}\\
B'_1&=\{\{2,3,i\}∈A|i≠2,j≠2\}\\
B'_2&=\{\{1,3,i\}∈A|i≠1,j≠1\}\\
B'_3&=\{\{1,2,i\}∈A|i≠3,j≠3\}\\
B_4&= \{\{a,b,c\}∈A|\{a,b,c\}∩\{1,2,3\}=∅\}
\end{align*}
Note that every vertex in $A$, other than $v$, belongs to exactly one of these sets.

Any element of $B_4$ can only belong to members of $S_2(A)$ since they have distance $3$ from $v$ and thus no common neighbours.

An element of $B_1$ can be a member of at most $4$ elements of $S_1$ since $v$ only shares $4$ neighbours with every element of $B_1$ that is to say those characterised by:
\begin{align*}
\{1,2,i\}\\
\{1,2,j\}\\ 
\{1,3,i\}\\  
\{1,3,j\}\\
\end{align*}

Similarly every element of $B_2$ and $B_3$ is a member of at most $4$  elements of $S_1$.
Note that as subsets of $A$, the size of $B_1,B_2$ and $B_3$ are linearly bounded in $|A|$.

An element of $B'_3$ has  $(m-3)+2$ neighbours in common with $v$.
They are 
$\{1,i,3\}$,
$\{i,2,3\}$,
and  $\{1,2,j\}$ for some $i$ where $j≠3$ and $j≠i$.


We want to find out how many vertices of the form $\{1,2,j\}$ have neighbourhoods that are distinct when intersected with $A$.
We start by  counting every vertex $u∈A$ of the form $\{1,2,j\}$ there are $|B'_3|≤n$  of those.

Note that any vertex of the form $\{1,2,j\}$ such that $N(\{1,2,j\})∩(B_1∪B_2∪B_3)≠∅$ has already been counted.
Thus we can assume that for all the remaining cases that $N(\{1,2,j\})∩(B_1∪B_2∪B_3)=∅$.

Let $u,w∉A$ be vertices of the form $\{1,2,j\}$. 
If $N(u)∩(B'_1∪B'_2)=∅$ and $N(w)∩(B'_1∪B'_2)=∅$  then $N(u)∩A=N(w)∩A=B'_3$.
Since any element of $B'_1∪B'_2$ has at most $1$ neighbour of the form $\{1,2,j\}$ this gives us at most $|B'_1∪B'_2|≤n$ sets.
Note that any two vertices in $B'_1$  will belong to the same neighbourhoods of this type  so we need not count them more than once.
Therefore the total number of sets in $S_1(A)$ obtained this way is $|B'_1∪B'_2|+|B'_3|≤n$.

Similarly the the number of sets in $S_1(A)$ obtained from $B'_1$ and $B'_2$ is less than $n$.
 

 
So now have a bound on the size of every part of  $S_1(A)$ and can compute a bound for $S(A)$.

\begin{align*}
&|S(A)|=\\
&|S_1(A)|+|S_2(A)|≤\\
&4n+3n+(4(n-1)^2)=\\
&7n+4(n^2-2n+1)=\\
&4n^2-n+1≤4n^2
\end{align*}

\end{proof}
\end{theorem}




==> Johnson/Density/InductionGeneralK.tex <==
\begin{theorem}
The shatter function $π(n)$ for the edge relation in $J(m,k)$ satisfies

$$π(n)≤4n+\min(m,n+1)\min(k,n+1)+π(n-1)$$

\begin{proof}

Let 
%$J(m,3)$ , with $m$ arbitrarily large.
$|A|=n$ be a set of vertices which is maximally shattered for sets of size $n$.
Let
$v∈A$
\begin{align*} 
S(A)&=\{N(u)∩A|u∈V(G)\}\\
S_1(A) &= \{ X∈ S(A): v∈X\}\\
S_2(A) &= \{ X∈ S(A): v∉X\}\\
\end{align*}
Note that $S(A)=S_1(A)∪S_2(A)$. 


%We prove the theorem by induction on $n$.
%Base case:
%We know by lemma \ref{SauerShelah} and theorem \ref{Johnson\VCDim} that $π{n}=2^n$ for  $n≤4$.
%$π(4)=2^4≤4\cdot 4^2$.

%Induction hypothesis:
%$$π(n-1)≤4(n-1)^2=4n^2-8n+4$$

%Inductive step:
Note that by our assumption that $A$ is maximally shattered we have  $|S(A)|= π(n)$.  
Since $S_2(A)=S(A∖\{v\})$ we know that $|S_2(A)|≤π(n-1)$.%as per induction hypothesis


Note that every member of  
$S_1(A)$ is an intersection of the neighbourhood of a neigbour of $v$ and $A$.
As these neighbours fully characterise each member of $S_1(A)$ we will use them evenhandedly to refer to
members of $S_1(A)$.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
We want count how many sets there are in $S_1(A)$. 
We do this by counting how many distinct neighbourhoods a given vertex in $A$ can occur in with $v$ and adding up over $A$.
This gives us a very loose upper bound which is sufficient for our purposes.
 


Let
\begin{align*} 
D_0&=\{v\}\\
D_1&=\{u∈A,d(u,v)=1\}\\
D_2&=\{u∈A,d(u,v)=2\}\\
D_3&=\{u∈A,d(u,v)≥3\}
\end{align*}
Note that $⋃_{i=0}^3D_i=A$ and for $i≠j$ we have $D_i∩D_j=∅$.

Any element of $D_3$ can only belong to members of $S_2(A)$ since they have  no common neighbours with $v$.

An element of $D_2$ can be a member of at most $4$ elements of $S_1(A)$ since $v$ only shares $4$ neighbours with every element of $D_2$.
Since $D_2⊆A$ we have $|D_2|≤|A|$,
%Note that as subsets of $A$, the size of $D_2$ is linearly bounded by $|A|$.
so the total number of sets in $S_1(A)$ that intersect $D_2$ is at most $4|A|$.

It only remains to count those sets in $S_1(A)$ that intersect $A$ only in $D_1$.

Since $D_1=N(v)∩A$ and any set in $S_1(v)$ must be characterised by a vertex in $N(v)$ 
we know that the number of sets in $S_1(v)$ contained in $D_1$ is bounded above by 
the shatter function $π'(n)$ for the edge relation in the $m$ by $k$ rook graph which by Lemma \ref{rook}
is bounded by $\min(i+1,n)\min(i+1,m)$.
 
$D_0$ is a singleton and its element $v$ is common to all members of $S_1(A)$ and it can therefore not distinguish any two members of $S_1(A)$.
So it adds no new sets to $S_1(A)$ unless $D_1=D_2=∅$.

 
So we  now have a bound on the size of every part of  $S_1(A)$ and can compute a bound for $S(A)$.

\begin{align*}
&π(n)=|S(A)|=\\
&|S_1(A)|+	|S_2(A)|≤\\
&0+4|A|+π'(n)+π(n-1)=\\
%&0+4|D_1|+π'(n)+π(n-1)=\\
&4n+\min(n+1,k)\min(n+1,m)+π(n-1)\\
\end{align*}

\end{proof}
\end{theorem}




==> Johnson/Density/Rook.tex <==
\begin{lemma}
\label{rook}
The shatter function $π(i)$ of the edge relation in the rook graph $R(n,m)$ is:
$$π(i)≤\min(i+1,n)\min(i+1,m)$$


\begin{proof}
Let $(R_j)_{j=1}^n$ and $(C_j)_{j=1}^m$ be the "rows" and "columns", respectively, of the rook graph.
Note that $R_j$ and $C_j$ are maximal cliques in the graph. 
Let $\mathcal{S}$ be the class of all neighbourhoods in the graph.
Moreover for any $1≤j≤n$ and $1≤k≤m$, the set $R_j∩C_k$ is a singleton. 
We will represent the vertex in that singleton by the pair $(j,k)$.
Note furthermore that every vertex is represented by  a unique pair in this way.

We now have that $N((j,k))=(R_j∪C_k)∖\{(j,k)\}$.


Now let $A$ be a set of vertices such that $|A|=i$ and $π(i)=|\{ A∩S|S∈\mathcal{S} \}|$.

There are now at most $i$ rows $R_j$ such that $A∩R_j≠∅$ and at most $i$ columns $C_j$ such that $A∩C_j≠∅$.
Every vertex $v$ that shares neither a row nor a column with any vertex of $A$ has $N(v)∩A=∅$.
We can by relabeling  guarantee that
any vertex $v=(j,k)$ such that $N(v)∩A≠∅$ must satisfy either 
$j≤i$ or  $k≤i$.

Note that there are  $\min(i,n)\min(i,m)$ vertices that satisfy both of those condititons and therefore at most $\min(i,n)\min(i,m)$ subsets of $A$ defined.

If $j>i$ then we have  $N(v)=A∩C_k$ so there can be at most $\min(n,i)$ distinct subsets of $A$ defined by such vertices, one for each column. 
If $k>i$ then we have  $N(v)=A∩R_j$ so there can be at most $\min(m,i)$ distinct subsets of $A$ defined by such vertices, one for each row.% for all vertices in $C_j$ beyond the $i$-th row.


This gives us a bound of:
$\min(i,n)\min(i,m) + \min(i,n)+\min(i,m)+1$.

If a row or a column is a subset of $A$ it cannot be contained in the neighbourhood of any vertex so the above expression  can be simplified to  $\min(i+1,n)\min(i+1,m)$.


\end{proof}
\end{lemma}


==> Johnson/Dimension/Talning.tex <==
Rules for generating all of the cases for configuration of $n$ vertices up to isomorphism.

We use the following rules in our judgements 
$$x_i=x_j\Rightarrow a_i≠a_j$$
$$a_i=a_j\Rightarrow x_i≠x_j$$
$$x_i=x_j\Rightarrow (\forall k i≤k≤j \rightarrow x_i=x_k)$$
$$ i≤j \Rightarrow |\{k|x_i=x_k\}|≤|\{k|x_j=x_k\}|$$


\begin{align*}
&x_1=x_2∧x_1=x_3∧x_1=x_4∧x_2=x_3∧x_2=x_4∧x_3=x_4
 \\∧
&a_1=a_2∧a_1=a_3∧a_1=a_4∧a_2=a_3∧a_2=a_4∧a_3=a_4
\end{align*}


%\begin{theorem}

%\begin{align}
%x_1=x_2∧x_1=x_3∧x_1=x_4∧
%\end{align}
\begin{centering}
\begin{figure}
\begin{tikzpicture}[y=-1cm,x=-1cm]%[thick,baseline={([yshift=9ex]current bounding box.center)}]
\node (n)	at (0,0) {12};
\node (t)	at (5,1) {8};
\node (tt)	at (8,2) {4};
\node (ttt)	at (9,3) {I};
\node (ttf)	at (7,3) {3};
\node (ttft)	at (8,4) {II};
\node (ttff)	at (6,4) {III};
\node (tf)	at (2,2) {6};
\node (tft)	at (4,3) {4};
\node (tftt)	at (5,4) {1};
\node (tfttt)	at (6,5) {IV};
\node (tfttf)	at (4,5) {V};
\node (tftf)	at (3,4) {VI};
\node (tff)	at (1,3) {5};
\node (tfft)	at (3,5) {2};
\node (tfftt)	at (4,6) {VII};
\node (tfftf)	at (2,6) {1};
\node (tfftft)	at (3,7) {VIII};
\node (tfftff)	at (1,7) {IX};
\node (tfff)	at (0,4) {1};
\node (tffft)	at (1,5) {X};
\node (tffff)	at (-1,5) {XI};
\node (f)	at (-5,1) {6};
\node (ft)	at (-3,2) {3};
\node (ftt)	at (-2,3) {1};
\node (fttt)	at (-1,4) {XII};
\node (fttf)	at (-3,4) {XIII};
\node (ftf)	at (-5,3) {1};
\node (ftft)	at (-4,4) {XIV};
\node (ftff)	at (-6,4) {XV};
\node (ff)	at (-6,2) {XVI};
\path[-]
	(n)	edge node [above left ] {$x_1=x_2$} (t)
	(n)	edge node [above right] {$x_1≠x_2$} (f)
	(t)	edge node [above left ] {$x_1=x_3$} (tt)
	(t)	edge node [above right] {$x_1≠x_3$} (tf)
	(tt)	edge node [above left ] {$x_1=x_4$} (ttt)
	(tt)	edge node [above right] {$x_1≠x_4$} (ttf)
	(ttf)	edge node [above left ] {$a_1=a_4$} (ttft)
	(ttf)	edge node [above right] {$a_1≠a_4$} (ttff)
	(tf)	edge node [above left ] {$x_3=x_4$} (tft)
	(tf)	edge node [above right] {$x_3≠x_4$} (tff)
	(tft)	edge node [above left ] {$a_1=a_3$} (tftt)
	(tft)	edge node [above right] {$a_1≠a_3$} (tftf)
	(tftt)	edge node [above left ] {$a_2=x_4$} (tfttt)
	(tftt)	edge node [above right] {$a_2≠a_4$} (tfttf)
	(tff)	edge node [above left ] {$a_1=a_3$} (tfft)
	(tff)	edge node [above right] {$a_1≠a_3$} (tfff)
	(tfft)	edge node [above left ] {$a_1=a_4$} (tfftt)
	(tfft)	edge node [above right] {$a_1≠a_4$} (tfftf)
	(tfftf)	edge node [above left ] {$a_2=a_4$} (tfftft)
	(tfftf)	edge node [above right] {$a_2≠a_4$} (tfftff)
	(tfff)	edge node [above left ] {$a_3=a_4$} (tffft)
	(tfff)	edge node [above right] {$a_3≠a_4$} (tffff)
	(f)	edge node [above left ] {$a_1=a_2$} (ft)
	(f)	edge node [above right] {$a_1≠a_2$} (ff)
	(ft)	edge node [above left ] {$a_1=a_3$} (ftt)
	(ft)	edge node [above right] {$a_1≠a_3$} (ftf)
	(ftt)	edge node [above left ] {$a_1=a_4$} (fttt)
	(ftt)	edge node [above right] {$a_1≠a_4$} (fttf)
	(ftf)	edge node [above left ] {$a_3=a_4$} (ftft)
	(ftf)	edge node [above right] {$a_3≠a_4$} (ftff)
;                               
\end{tikzpicture}               
\end{figure}
\end{centering}



%\end{theorem}




==> Johnson/Dimension/tilfellin12.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%það eru 16 tilfelli af stærð 4
%I)	II)	III)	IV)	V)	VI)	VII)	VIII)	IX)	X)	XI)	XII)
%xx  	xx 	xx	xxx	xxx	xxxx	xx	x	x	x	x	x
%xx	 xx 	  xx	x	   x		x	xx	x	x	x	 x
%						x	 x	x	 x	x	  x
%								 x	 x	x	   x
%þau sem splundrast eru 1 5 6 7 8 12 14
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\begin{lemma}
%Let $v$ be a vertex in a johnson graph
%and let $w=v∖\{a,b\}∪\{x,y\}$ be a vertex such that $d(v,w)=2$
%then 
%for all $u∈(N(v)∩N(w))$ we have $u=v∖\{c\}∪\{z\}$ where $c∈\{a,b\}$ and $ z∈\{x,y\}$ 
%\end{lemma}
%
%\begin{lemma}
%Let $v$ be a vertex in a johnson graph
%and let $w=v∖\{a\}∪\{x\}$ be a vertex such that $d(v,w)=1$
%then 
%for all $u∈(N(v)∩N(w))$ we have $u=v∖\{c\}∪\{z\}$ where $c∈\{a\}$ or $ z∈\{x\}$ 
%\end{lemma}

%\input{Johnson/Talning.tex}

%Assume $|A|≥4$ let $v$ be such that $A⊆N(v)$
%we know that all $u$ in $A$ have the form $u=v∖\{a\}∪\{x\}$.


We now have $16$ cases and will go through them one by one demonstrating that in each case either
$A$ can not be shattered or that adding a fifth vertex to $A$ will always result in a set that cannot be shattered.


\begin{enumerate}[label=\textbf{Case \Roman*}]
\item
%I) shatters                           
%xxxx
%
%
%
\begin{multicols}{2}
\begin{align*}
	v_1 = v∖\{a_1\}∪\{x_1\}\\
	v_2 = v∖\{a_2\}∪\{x_1\}\\
	v_3 = v∖\{a_3\}∪\{x_1\}\\
	v_4 = v∖\{a_4\}∪\{x_1\}\\
\end{align*}
\begin{tikzpicture}[thick,baseline={([yshift=9ex]current bounding box.center)}]
\node[draw,circle] (A) at ( 0, 0) {$v_1$};
\node[draw,circle] (B) at ( 1, 0) {$v_2$};
\node[draw,circle] (C) at ( 2, 0) {$v_3$};
\node[draw,circle] (D) at ( 3, 0) {$v_4$};
\end{tikzpicture}
\end{multicols}

This Shatters, 
	so we need 
	\begin{enumerate}%[label=\alpha]
	\item
	$v_5 = v∖\{a_5\}∪\{x_1\}$
	Picking out a triple from $5$ in a row is impossible
	\item
	$v_5 = v∖\{a_1\}∪\{x_2\}$
	Here $v_1,v_2,v_3,v_5$ form case $II$ 
	\item
	$v_5 = v∖\{a_5\}∪\{x_2\}$
	Here $v_1,v_2,v_3,v_5$ 
	\end{enumerate}
%

\item
%II) shatters                          
%123
%4 
%
%
\begin{multicols}{3}
\begin{align*}
	v_1 = v∖\{a_1\}∪\{x_1\}\\
	v_2 = v∖\{a_2\}∪\{x_1\}\\
	v_3 = v∖\{a_3\}∪\{x_1\}\\
	v_4 = v∖\{a_1\}∪\{x_2\}\\
\end{align*}
\begin{tikzpicture}[thick,baseline={([yshift=9ex]current bounding box.center)}]
\node[draw,circle] (A) at ( 0, 0) {$v_1$};
\node[draw,circle] (B) at ( 1, 0) {$v_2$};
\node[draw,circle] (C) at ( 2, 0) {$v_3$};
\node[draw,circle] (D) at ( 0, 1) {$v_4$};
\end{tikzpicture}
\end{multicols}
This Shatters, 
	so we need 
	\begin{enumerate}%[label=\alpha]
	\item
	$v_5 = v∖\{a_2\}∪\{x_2\}$
	then $v_1,v_2,v_4,v_5$ forms case $IV$ 
	\item
	$v_5 = v∖\{a_4\}∪\{x_2\}$
	then $v_1,v_2,v_3,v_5$ forms case $III$ 
	\item
	$v_5 = v∖\{a_1\}∪\{x_3\}$
	then $v_2,v_3,v_4,v_5$ forms case $X$ 
	\item
	$v_5 = v∖\{a_2\}∪\{x_3\}$
	then $v_1,v_3,v_4,v_5$ forms case $IX$ 
	\item
	$v_5 = v∖\{a_4\}∪\{x_3\}$
	then $v_1,v_2,v_4,v_5$ forms case $IX$ 
	\end{enumerate}
		
		 

\item
%III)                            
%123
%   4
%
%
\begin{multicols}{3}
\begin{align*}
	v_1 = v∖\{a_1\}∪\{x_1\}\\
	v_2 = v∖\{a_2\}∪\{x_1\}\\
	v_3 = v∖\{a_3\}∪\{x_1\}\\
	v_4 = v∖\{a_4\}∪\{x_2\}\\
\end{align*}
\begin{tikzpicture}[thick,baseline={([yshift=9ex]current bounding box.center)}]
\node[draw,circle] (A) at ( 0, 0) {$v_1$};
\node[draw,circle] (B) at ( 1, 0) {$v_2$};
\node[draw,circle] (C) at ( 2, 0) {$v_3$};
\node[draw,circle] (D) at ( 3, 1) {$v_4$};
\end{tikzpicture}
\end{multicols}
	Let $w$ be such that
	 $w∩A=\{v_1,v_2,v_4\}$
	we have 2 cases 
		$w=v∖\{a\}∪\{x\}$ or
		since we have to exclude $v_1$ we must have that $a≠a_1$ and $x≠x_1$ 
		so in order to have $v_2∈N(w)$ we must  have $a=a_2$
		so in order to have $v_3∈N(w)$ we must  have $a=x_3$
		but then $a_2=a_3$  in contradiction with $v_1≠v_2$
		
		$w=v∖\{a,b\}∪\{x,y\}$ 
	  	    in order to have $v_2∈N(w)$ we must  have $a_2∈\{a,b\}$ and $x_1∈\{x,y\}$
		and in order to have $v_3∈N(w)$ we must  have $a_3∈\{a,b\}$ and $x_1∈\{x,y\}$
		and in order to have $v_4∈N(w)$ we must  have $a_4∈\{a,b\}$ and $x_2∈\{x,y\}$
		but then $\{a_2,a_3,a_4\}⊆\{a,b\}$ in contradiction with $3≥2$.


\item
%IV)
%12
%34
%
%
\begin{multicols}{3}
\begin{align*}
	v_1 = v∖\{a_1\}∪\{x_1\}\\
	v_2 = v∖\{a_1\}∪\{x_2\}\\
	v_3 = v∖\{a_2\}∪\{x_1\}\\
	v_4 = v∖\{a_2\}∪\{x_2\}\\
\end{align*}
\begin{tikzpicture}[thick,baseline={([yshift=9ex]current bounding box.center)}]
\node[draw,circle] (A) at ( 0, 0) {$v_1$};
\node[draw,circle] (B) at ( 1, 0) {$v_2$};
\node[draw,circle] (C) at ( 0, 1) {$v_3$};
\node[draw,circle] (D) at ( 1, 1) {$v_4$};
\end{tikzpicture}
\end{multicols}
	Let $w$ be such that  
	 $w∩A=\{v_3,v_3,v_4\}$

	we have 2 cases 
		$w=v∖\{a\}∪\{x\}$ or
		since we have to exclude $v_1$ we must have that $a≠a_1$ and $x≠x_1$ 
		so in order to have $v_2∈N(w)$ we must  have $a=a_2$
		so in order to have $v_3∈N(w)$ we must  have $x=x_2$
		but then $w=v_1$ in contradiction with $v_1∈N(w)$
		
		$w=v∖\{a,b\}∪\{x,y\}$ 
	  	    in order to have $v_2∈N(w)$ we must  have $a_1∈\{a,b\}$ and $x_2∈\{x,y\}$
		and in order to have $v_3∈N(w)$ we must  have $a_2∈\{a,b\}$ and $x_1∈\{x,y\}$
		so $w=v∖\{a_1,a_2\}∪\{x_1,x_2\}$ in contradiction with $v_1∉N(w)$

\item
%V) splundrast
%12
% 34
%
%
\begin{multicols}{3}
\begin{align*}
	v_1 = v∖\{a_1\}∪\{x_1\}\\
	v_2 = v∖\{a_2\}∪\{x_1\}\\
	v_3 = v∖\{a_2\}∪\{x_2\}\\
	v_4 = v∖\{a_3\}∪\{x_2\}\\
\end{align*}
\begin{tikzpicture}[thick,baseline={([yshift=9ex]current bounding box.center)}]
\node[draw,circle] (A) at ( 0, 0) {$v_1$};
\node[draw,circle] (B) at ( 1, 0) {$v_2$};
\node[draw,circle] (C) at ( 1, 1) {$v_3$};
\node[draw,circle] (D) at ( 2, 1) {$v_4$};
\end{tikzpicture}
\end{multicols}
	\begin{enumerate}%[label=\alpha]
	\item
	$v_5 = v∖\{a_1\}∪\{x_3\}$
	Here $v_2,v_4,v_5$ form the diagonal
	\item
	$v_5 = v∖\{a_2\}∪\{x_3\}$
	Here $v_1,v_4,v_5$ form the diagonal
	\item
	$v_5 = v∖\{a_3\}∪\{x_3\}$
	Here $v_2,v_3,v_5$ form the diagonal
	\item
	$v_5 = v∖\{a_4\}∪\{x_3\}$
	In this case $v_2,v_3,v_5$ form the diagonal
	\end{enumerate}

\item
%VI) splundrast
%12
%  34
%
%
\begin{multicols}{3}
\begin{align*}
	v_1 = v∖\{a_1\}∪\{x_1\}\\
	v_2 = v∖\{a_2\}∪\{x_1\}\\
	v_3 = v∖\{a_3\}∪\{x_2\}\\
	v_4 = v∖\{a_4\}∪\{x_2\}\\
\end{align*}
\begin{tikzpicture}[thick,baseline={([yshift=9ex]current bounding box.center)}]
\node[draw,circle] (A) at ( 0, 0) {$v_1$};
\node[draw,circle] (B) at ( 1, 0) {$v_2$};
\node[draw,circle] (C) at ( 2, 1) {$v_3$};
\node[draw,circle] (D) at ( 3, 1) {$v_4$};
\end{tikzpicture}
\end{multicols}
	\begin{enumerate}%[label=\alpha]
	\item
	$v_5 = v∖\{a_1\}∪\{x_3\}$
	In this case $v_1,v_3,v_4,v_5$ form case $X$
	\item
	$v_5 = v∖\{a_2\}∪\{x_3\}$
	In this case $v_2,v_3,v_4,v_5$ form case $X$
	\item
	$v_5 = v∖\{a_3\}∪\{x_3\}$
	In this case $v_1,v_2,v_3,v_5$ form case $X$
	\item
	$v_5 = v∖\{a_4\}∪\{x_3\}$
	In this case $v_1,v_2,v_4,v_5$ form case $X$
	\item
	$v_5 = v∖\{a_5\}∪\{x_3\}$
	In this case $v_1,v_3,v_5$ form the diagonal
	\end{enumerate}

\item
%VII) splundrast                
%12 
%3
%4
%
\begin{multicols}{3}
\begin{align*}
	v_1 = v∖\{a_1\}∪\{x_1\}\\
	v_2 = v∖\{a_1\}∪\{x_2\}\\
	v_3 = v∖\{a_1\}∪\{x_3\}\\
	v_4 = v∖\{a_2\}∪\{x_1\}\\
\end{align*}
\begin{tikzpicture}[thick,baseline={([yshift=9ex]current bounding box.center)}]
\node[draw,circle] (A) at ( 0, 0) {$v_1$};
\node[draw,circle] (B) at ( 1, 0) {$v_2$};
\node[draw,circle] (C) at ( 0, 1) {$v_3$};
\node[draw,circle] (D) at ( 0, 2) {$v_4$};
\end{tikzpicture}
\end{multicols}
	\begin{enumerate}%[label=\alpha]
	\item
	$v_5 = v∖\{a_1\}∪\{x_4\}$
	Here $v_2,v_3,v_4,v_5$ form case $XIII$ 
	\item
	$v_5 = v∖\{a_2\}∪\{x_4\}$
	In this case $v_1,v_3,v_4,v_5$ form case $XIII$
	\item
	$v_5 = v∖\{a_3\}∪\{x_4\}$
	In this case $v_1,v_3,v_4,v_5$ form case $XIII$	
	\end{enumerate}
%
%
\item
%VIII) splundrast
%12
%3
% 4
%
\begin{multicols}{3}
\begin{align*}
	v_1 = v∖\{a_1\}∪\{x_1\}\\
	v_2 = v∖\{a_2\}∪\{x_1\}\\
	v_3 = v∖\{a_1\}∪\{x_2\}\\
	v_4 = v∖\{a_2\}∪\{x_3\}\\
\end{align*}
\begin{tikzpicture}[thick,baseline={([yshift=9ex]current bounding box.center)}]
\node[draw,circle] (A) at ( 0, 0) {$v_1$};
\node[draw,circle] (B) at ( 1, 0) {$v_2$};
\node[draw,circle] (C) at ( 0, 1) {$v_3$};
\node[draw,circle] (D) at ( 1, 2) {$v_4$};
\end{tikzpicture}
\end{multicols}
	\begin{enumerate}%[label=\alpha]
	\item
	$v_5 = v∖\{a_1\}∪\{x_4\}$
	In this case $v_1,v_3,v_4,v_5$ form case $XIII$
	\item
	$v_5 = v∖\{a_2\}∪\{x_4\}$
	Here $v_2,v_3,v_4,v_5$ form case $XIII$ 
	\item
	$v_5 = v∖\{a_3\}∪\{x_4\}$
	In this case $v_3,v_4,v_5$ form the diagonal
	\end{enumerate}

\item
%IX)
%12
%3
%  4
\begin{multicols}{3}
\begin{align*}
	v_1 = v∖\{a_1\}∪\{x_1\}\\
	v_2 = v∖\{a_2\}∪\{x_1\}\\
	v_3 = v∖\{a_1\}∪\{x_2\}\\
	v_4 = v∖\{a_3\}∪\{x_3\}\\
	 w∩A=\{v_2,v_3,v_4\}
\end{align*}
\begin{tikzpicture}[thick,baseline={([yshift=9ex]current bounding box.center)}]
\node[draw,circle] (A) at ( 0, 0) {$v_1$};
\node[draw,circle] (B) at ( 1, 0) {$v_2$};
\node[draw,circle] (C) at ( 0, 1) {$v_3$};
\node[draw,circle] (D) at ( 2, 2) {$v_4$};
\end{tikzpicture}
\end{multicols}
	Let $w$ be such that  
	 $w∩A=\{v_2,v_3,v_4\}$
	we have 2 cases
 
		$w=v∖\{a\}∪\{x\}$: 
		in order to have $v_2∈N(w)$ and $v_3∈N(w)$ we must  have $a=a_2∧x=x_3$ or $a=a_3∧x=x_2$
		but both cases we have   $v_4∉N(w)$ in contradiction with our assumptions
		
		$w=v∖\{a,b\}∪\{x,y\}$: 
	  	    in order to have $v_2∈N(w)$ we must  have $a_2∈\{a,b\}$ and $x_2∈\{x,y\}$
		and in order to have $v_3∈N(w)$ we must  have $a_3∈\{a,b\}$ and $x_3∈\{x,y\}$
		so $w=v∖\{a_2,a_3\}∪\{x_2,x_3\}$ in contradiction with $v_4∈N(w)$


\item
%X)
%12
%  3
%  4
\begin{multicols}{3}
\begin{align*}
	v_1 = v∖\{a_1\}∪\{x_1\}\\
	v_2 = v∖\{a_2\}∪\{x_1\}\\
	v_3 = v∖\{a_3\}∪\{x_2\}\\
	v_4 = v∖\{a_3\}∪\{x_3\}\\
	 w∩A=\{v_2,v_3,v_4\}
\end{align*}
\begin{tikzpicture}[thick,baseline={([yshift=9ex]current bounding box.center)}]
\node[draw,circle] (A) at ( 0, 0) {$v_1$};
\node[draw,circle] (B) at ( 1, 0) {$v_2$};
\node[draw,circle] (C) at ( 2, 1) {$v_3$};
\node[draw,circle] (D) at ( 2, 2) {$v_4$};
\end{tikzpicture}
\end{multicols}
%diagonal
	Let $w$ be such that  
	 $w∩A=\{v_2,v_3,v_4\}$
	we have 2 cases
 
		since we have to exclude $v_1$ we must have that $a≠a_1$ and $x≠x_1$ 
		so in order to have $v_2∈N(w)$ we must  have $a=a_2$
		so in order to have $v_3∈N(w)$ we must  have $x=x_2$
		but then $w=v∖\{a_2\}∪\{x_2\}$  in contradiction with $v_4∈N(w)$
%		
		$w=v∖\{a,b\}∪\{x,y\}$ 
	  	    in order to have $v_2∈N(w)$ we must  have $a_2∈\{a,b\}$ and $x_1∈\{x,y\}$
		and in order to have $v_3∈N(w)$ we must  have $a_3∈\{a,b\}$ and $x_2∈\{x,y\}$
		so $w=v∖\{a_2,a_3\}∪\{x_1,x_2\}$ in contradiction with $v_4∉N(w)$


\item
%XI)
%12
%  3
%   4
%
\begin{multicols}{3}
\begin{align*}
	v_1 = v∖\{a_1\}∪\{x_1\}\\
	v_2 = v∖\{a_2\}∪\{x_1\}\\
	v_3 = v∖\{a_3\}∪\{x_2\}\\
	v_4 = v∖\{a_4\}∪\{x_3\}\\
	 w∩A=\{v_2,v_3,v_4\}
\end{align*}
\begin{tikzpicture}[thick,baseline={([yshift=9ex]current bounding box.center)}]
\node[draw,circle] (A) at ( 0, 0) {$v_1$};
\node[draw,circle] (B) at ( 1, 0) {$v_2$};
\node[draw,circle] (C) at ( 2, 1) {$v_3$};
\node[draw,circle] (D) at ( 3, 2) {$v_4$};
\end{tikzpicture}
\end{multicols}
%diagonal
	Let $w$ be such that  
	 $w∩A=\{v_2,v_3,v_4\}$
	we have 2 cases
 
		$w=v∖\{a\}∪\{x\}$: 
		in order to have $v_2∈N(w)$ and $v_3∈N(w)$ we must  have $a=a_2∧x=x_3$ or $a=a_3∧x=x_2$
		but both cases we have   $v_4∉N(w)$ in contradiction with our assumptions
		
		$w=v∖\{a,b\}∪\{x,y\}$: 
	  	    in order to have $v_2∈N(w)$ we must  have $a_2∈\{a,b\}$ and $x_2∈\{x,y\}$
		and in order to have $v_3∈N(w)$ we must  have $a_3∈\{a,b\}$ and $x_3∈\{x,y\}$
		so $w=v∖\{a_2,a_3\}∪\{x_2,x_3\}$ in contradiction with $v_4∈N(w)$

\item
%XII) splundrast
%1
%2
%3
%4
\begin{multicols}{3}
\begin{align*}
	v_1 = v∖\{a_1\}∪\{x_1\}\\
	v_2 = v∖\{a_1\}∪\{x_2\}\\
	v_3 = v∖\{a_2\}∪\{x_3\}\\
	v_4 = v∖\{a_3\}∪\{x_4\}\\
	 w∩A=\{v_2,v_3,v_4\}
\end{align*}
\begin{tikzpicture}[thick,baseline={([yshift=9ex]current bounding box.center)}]
\node[draw,circle] (A) at (0 , 0) {$v_1$};
\node[draw,circle] (B) at (0 , 1) {$v_2$};
\node[draw,circle] (C) at (0 , 2) {$v_3$};
\node[draw,circle] (D) at (0 , 3) {$v_4$};
\end{tikzpicture}
\end{multicols}
	\begin{enumerate}%[label=\alpha]
	\item
	$v_5 = v∖\{a_1\}∪\{x_5\}$
	Picking out a triple from $5$ in a row is impossible
	\item
	$v_5 = v∖\{a_2\}∪\{x_5\}$	
	Here $v_2,v_3,v_4,v_5$ form case $XIII$ 
	\end{enumerate}

\item
%XIII)
%1
%2
%3
% 4
\begin{multicols}{3}
\begin{align*}
	v_1 = v∖\{a_1\}∪\{x_1\}\\
	v_2 = v∖\{a_1\}∪\{x_2\}\\
	v_3 = v∖\{a_1\}∪\{x_3\}\\
	v_4 = v∖\{a_2\}∪\{x_4\}\\
	 w∩A=\{v_2,v_3,v_4\}
\end{align*}
\begin{tikzpicture}[thick,baseline={([yshift=9ex]current bounding box.center)}]
\node[draw,circle] (A) at (0 , 0) {$v_1$};
\node[draw,circle] (B) at (0 , 1) {$v_2$};
\node[draw,circle] (C) at (0 , 2) {$v_3$};
\node[draw,circle] (D) at (1 , 3) {$v_4$};
\end{tikzpicture}
\end{multicols}
	Let $w$ be such that  
	 $w∩A=\{v_1,v_2,v_3\}$
	 %w∩A=\{v_2,v_3,v_4\}
	
	we have 2 cases 
		$w=v∖\{a\}∪\{x\}$ or
		since we have to exclude $v_1$ we must have that $a≠a_1$ and $x≠x_1$ 
		so in order to have $v_2∈N(w)$ we must  have $x=x_1$
		so in order to have $v_3∈N(w)$ we must  have $x=x_3$
		but then $x_2=x_3$  in contradiction with $v_1≠v_2$
%		
		$w=v∖\{a,b\}∪\{x,y\}$ 
	  	    in order to have $v_2∈N(w)$ we must  have $a_1∈\{a,b\}$ and $x_2∈\{x,y\}$
		and in order to have $v_3∈N(w)$ we must  have $a_1∈\{a,b\}$ and $x_3∈\{x,y\}$
		and in order to have $v_4∈N(w)$ we must  have $a_2∈\{a,b\}$ and $x_4∈\{x,y\}$
		but then $\{x_2,a_3,a_4\}⊆\{x,y\}$ in contradiction with $3≥2$.

\item
%XIV) splundrast
%1
%2
% 3
% 4
\begin{multicols}{3}
\begin{align*}
	v_1 = v∖\{a_1\}∪\{x_1\}\\
	v_2 = v∖\{a_1\}∪\{x_2\}\\
	v_3 = v∖\{a_2\}∪\{x_3\}\\
	v_4 = v∖\{a_2\}∪\{x_4\}\\
	 w∩A=\{v_2,v_3,v_4\}
\end{align*}
\begin{tikzpicture}[thick,baseline={([yshift=9ex]current bounding box.center)}]
\node[draw,circle] (A) at (0 , 0) {$v_1$};
\node[draw,circle] (B) at (0 , 1) {$v_2$};
\node[draw,circle] (C) at (1 , 2) {$v_3$};
\node[draw,circle] (D) at (1 , 3) {$v_4$};
\end{tikzpicture}
\end{multicols}
	\begin{enumerate}%[label=\alpha]
	\item
	$v_5 = v∖\{a_1\}∪\{x_5\}$
	In this case $v_1,v_2,v_5,v_3$ form case $XIII$
	\item
	$v_5 = v∖\{a_2\}∪\{x_5\}$
	In this case $v_2,v_4,v_5,v_3$ form case $XIII$
	\item
	$v_5 = v∖\{a_3\}∪\{x_5\}$
	Here $v_3,v_4,v_5$ form the diagonal
	\end{enumerate}




\item
%XV)
%1
%2
% 3
%  4
\begin{multicols}{3}
\begin{align*}
	v_1 = v∖\{a_1\}∪\{x_1\}\\
	v_2 = v∖\{a_1\}∪\{x_2\}\\
	v_3 = v∖\{a_2\}∪\{x_3\}\\
	v_4 = v∖\{a_3\}∪\{x_4\}\\
	 w∩A=\{v_2,v_3,v_4\}
\end{align*}
\begin{tikzpicture}[thick,baseline={([yshift=9ex]current bounding box.center)}]
\node[draw,circle] (A) at (0 , 0) {$v_1$};
\node[draw,circle] (B) at (0 , 1) {$v_2$};
\node[draw,circle] (C) at (1 , 2) {$v_3$};
\node[draw,circle] (D) at (2 , 3) {$v_4$};
\end{tikzpicture}
\end{multicols}
%diagonal

	Let $w$ be such that  
	 $w∩A=\{v_2,v_3,v_4\}$
	we have 2 cases
 
		$w=v∖\{a\}∪\{x\}$: 
		in order to have $v_2∈N(w)$ and $v_3∈N(w)$ we must  have $a=a_2∧x=x_3$ or $a=a_3∧x=x_2$
		but both cases we have   $v_4∉N(w)$ in contradiction with our assumptions
		
		$w=v∖\{a,b\}∪\{x,y\}$: 
	  	    in order to have $v_2∈N(w)$ we must  have $a_2∈\{a,b\}$ and $x_2∈\{x,y\}$
		and in order to have $v_3∈N(w)$ we must  have $a_3∈\{a,b\}$ and $x_3∈\{x,y\}$
		so $w=v∖\{a_2,a_3\}∪\{x_2,x_3\}$ in contradiction with $v_4∈N(w)$
\item
%XVI)
%1
% 2
%  3
%   4
\begin{multicols}{3}
\begin{align*}
	v_1 = v∖\{a_1\}∪\{x_1\}\\
	v_2 = v∖\{a_2\}∪\{x_2\}\\
	v_3 = v∖\{a_3\}∪\{x_3\}\\
	v_4 = v∖\{a_4\}∪\{x_4\}\\
	 w∩A=\{v_2,v_3,v_4\}
\end{align*}
\begin{tikzpicture}[thick,baseline={([yshift=9ex]current bounding box.center)}]
\node[draw,circle] (A) at (0 , 0) {$v_1$};
\node[draw,circle] (B) at (1 , 1) {$v_2$};
\node[draw,circle] (C) at (2 , 2) {$v_3$};
\node[draw,circle] (D) at (3 , 3) {$v_4$};
\end{tikzpicture}
\end{multicols}
%diagonal
	Let $w$ be such that  
	 $w∩A=\{v_2,v_3,v_4\}$
	we have 2 cases
 
		$w=v∖\{a\}∪\{x\}$: 
		in order to have $v_2∈N(w)$ and $v_3∈N(w)$ we must  have $a=a_2∧x=x_3$ or $a=a_3∧x=x_2$
		but both cases we have   $v_4∉N(w)$ in contradiction with our assumptions
		
		$w=v∖\{a,b\}∪\{x,y\}$: 
	  	    in order to have $v_2∈N(w)$ we must  have $a_2∈\{a,b\}$ and $x_2∈\{x,y\}$
		and in order to have $v_3∈N(w)$ we must  have $a_3∈\{a,b\}$ and $x_3∈\{x,y\}$
		so $w=v∖\{a_2,a_3\}∪\{x_2,x_3\}$ in contradiction with $v_4∈N(w)$

\end{enumerate}


==> Johnson/Lemmas/Lemmas.tex <==
\TODO[Uppfæra sannanir fyrir Symmetric difference]
\subsection{Properties of Johnson Graphs}
%\TODO[Skilgreiningar og dót hér er farið beint í afleiðingu]
\begin{lemma}
\label{d1}
Let $v$ and $w$ be vertices in a Johnson graph with
$d(v,w)=1$.
Write 
$w=(v∖\{a\})∪\{x\}$.
Then we have
$u∈N(v)∩N(w)$
if and only if
$u=(v∖\{c\})∪\{z\}$
with 
$
(c=a)
\oplus
(z=x)
$.

\begin{proof}

Assume $u∈N(v)∩N(w)$ then since $d(v,u)=1$ we must have
$u=v∖\{c\}∪\{z\}$ for some $c$ and $T$.
Now assume $c≠a$ and $z≠x$ then we have 
$u\Delta w=\{a,c,x,z\}$
so $|u\Delta v|=4$ in contradiction with $d(u,w)=1$.
So we must have $c=a$ or $z=x$

Assume $u=v∖\{a\}∪\{z\}$ with $x≠z$. 
Then 
$u∩v=v∖\{a\}$ which has size $k-1$ so $u∈N(v)$.
Also
$u∩w=v∖\{a\}$ which has size $k-1$ so $u∈N(w)$.
Thus we have $u∈N(v)∩N(w)$.


Assume $u=v∖\{c\}∪\{x\}$ then 
$u∩v=v∖\{c\}$ which has size $k-1$ so $u∈N(v)$.
Also
$u∩w=v∖\{a,c\}∪\{x\}$ which has size $k-1$ so $u∈N(w)$.
Thus we have $u∈N(v)∩N(w)$.


Note that if we have both $c=a$ and $z=x$ then $u=w$ in contradiction with $Euw$.
\end{proof}
\end{lemma}

\begin{lemma}
\label{d2}
Let $v$ and $w$ be a vertices in a Johnson graph with
$d(v,w)=2$.
We can write $w=v∖\{a,b\}∪\{x,y\}$.
Then we have 
$u∈N(v)∩N(w)$
if and only if
$u=v∖\{c\}∪\{z\}$
with $c∈\{a,b\}∧z∈\{x,y\}$.
\begin{proof}
Assume $u∈N(v)∩N(w)$ .Then since $d(v,u)=1$ we must have
$u=v∖\{c\}∪\{z\}$ for some $c∈v$ and $z∉v$.

Now assume $c∉\{a,b\}$.
Then we have 
$u\Delta w⊇\{a,b,c\}$ in contradiction with $|u\Delta w|=2$.

Assume
$z∉\{x,y\}$.
Then we have 
$u\Delta w⊇\{x,y,z\}$ in contradiction with $|u\Delta w|=2$.
So we must have $c∈\{a,b\}∧z∈\{x,y\}$.

Now assume $u=v∖\{c\}∪\{z\}$ with  $c∈\{a,b\}∧z∈\{x,y\}$.
Assume without loss of generality $u=v∖\{a\}∪\{x\}$ then 
$u∩v=v∖\{a\}$ which has size $k-1$ so $u∈N(v)$.
Also
$u∩w=v∖\{a,b\}∪\{x\}$ which has size $k-1$ so $u∈N(w)$ 
so we have $u∈N(v)∩N(w)$.
\end{proof}
\end{lemma}






\begin{lemma}
Let $A$ be set of vertices in Johnson graph shattered by the edge relation and assume $A≥4$. % $v$ be a vertex such that $A⊆N(v)$.

Then there do not exist $3$ vertices in $A$ each at distance $2$ from each other.
\label{Diag} 
\begin{proof}
%Let $v^a_x:=v∖\{a\}∪\{x\}$

Let $v$ be a vertex such that $A⊆N(v)$ and $A$ contains three vertices that are pairwise of distance $2$ from each other.

That is to say we have  
%$v_a^x,v_b^y,v_c^z∈A$ 
$$
\substack{
v∖\{a\}∪\{x\}∈A\\
v∖\{b\}∪\{y\}∈A\\
v∖\{c\}∪\{z\}∈A\\
}
$$ where $a,b,c,x,y,z$ are all distinct. 

Let $w$ be a vertex such that 
$N(w)∩A=\{
%v_a^x,v_b^y,v_c^z
v∖\{a\}∪\{x\},v∖\{b\}∪\{y\},v∖\{c\}∪\{z\}
\}$.

If $d(v,w)=1$ we can write $w=v∖\{a_1\}∪\{x_1\}$ by Lemma \ref{d1}.
We know that 
since $v∖\{a\}∪\{x\}∈N(w)$ we have $a_1=a∨x_1=x$ 

	Assume $a_1 = a$ then since $v∖\{b\}∪\{y\}∈N(w)$ we must have $x_1=y$, 
	so we have $w=v∖\{a\}∪\{y\}$.
	However
	$v∖\{c\}∪\{z\}∉N(v∖\{a\}∪\{y\})$ in contradiction to  
	$N(w)∩A=\{
v∖\{a\}∪\{x\},v∖\{b\}∪\{y\},v∖\{c\}∪\{z\}
%v_a^x,v_b^y,v_c^z
\}$.

	Assume $x_1 = y$ then since $v∖\{b\}∪\{y\}∈N(w)$
	we have  $a_1=b$ so we have $w=v∖\{b\}∪\{x\}$.
	However
	$v∖\{c\}∪\{z\}∉N(v∖\{b\}∪\{x\})$ in contradiction to  
	$N(w)∩A=\{
v∖\{a\}∪\{x\},v∖\{b\}∪\{y\},v∖\{c\}∪\{z\}
%v_a^x,v_b^y,v_c^z
\}$.


So we must have $d(v,w)=2$ and write $w=v∖\{a_1,a_2\}∪\{x_1,x_2\}$ by lemma \ref{d2} we know that
since $v∖\{a\}∪\{x\}∈N(w)$ we have $a∈\{a_1,a_2\}∧x∈\{x_1,x_2\}$.
 Without loss of generality we assume $a_1=a∧x_1=x$.

Similarily we have
 $v∖\{b\}∪\{y\}∈N(w)$ we have $b∈\{a,a_2\}∧y∈\{x,x_2\}$ 
so we have $w=v∖\{a,b\}∪\{x,y\}$ but then $v∖\{c\}∪\{z\}∉N(w)$ in contradiction with 
	$N(w)∩A=\{
%v_a^x,v_b^y,v_c^z
v∖\{a\}∪\{x\},v∖\{b\}∪\{y\},v∖\{c\}∪\{z\}
\}$

So there exists no $w$ for which 
	$N(w)∩A=\{
%v_a^x,v_b^y,v_c^z
v∖\{a\}∪\{x\},v∖\{b\}∪\{y\},v∖\{c\}∪\{z\}
\}$
	in contradiction with $A$ being shattered by the edge relation.
%Therefore we have that if $|A|≤4$ then for each vertex $u∈A$  we can have at most $1$ vertex of distance $2$ from $u$.
\end{proof}
\end{lemma}

\begin{lemma}
\label{JohnsonIndSub}
$J(n-1,k-1)$ is an induced subgraph of $J(n,k)$ 
\begin{proof}
Let $X$ be the underlying set for $J(n,k)$.
Let $x∈X$ and $V_x=\{v∈V(J(n,k)| x∈v \}$.
Let $f(v)=v∖\{x\}$ be a map from $V_x$ to $V(J(n-1,k-1)$ and $id(v)=v$ be a map from $V(J(n,k)∖V_x$.

Note that these maps are graph isomorphisms from the subgraphs induced by their preimage to their respective images.

%Observe that $f$ is an isomorphism from $J(n,k)[V_x]$ to $J(n-1,k-1)$ and $\id$ is an isomorphism from $J(n,k)[V(J(n,k))∖V_x]$ to $J(n-1,k)$ 


\end{proof}
\end{lemma}





